Easy-to-Hard: Leveraging Simple Questions for Complex Question Generation

This paper makes one of the first efforts toward automatically generating complex questions from knowledge graphs. Particularly, we study how to leverage existing simple question datasets for this task, under two separate scenarios: using either sub-questions of the target complex questions, or distantly related pseudo sub-questions when the former are unavailable. First, a competitive base model named CoG2Q is designed to map complex query qraphs to natural language questions. Afterwards, we propose two extension models, namely CoGSub2Q and CoGSub^m2Q, respectively for the above two scenarios. The former encodes and copies from a sub-question, while the latter further scores and aggregates multiple pseudo sub-questions. Experiment results show that the extension models significantly outperform not only base CoG2Q, but also its augmented variant using simple questions as additional training examples. This demonstrates the importance of instance-level connections between simple and corresponding complex questions, which may be underexploited by straightforward data augmentation of CoG2Q that builds model-level connections through learned parameters.

==> sections/experiment.tex <==

\section{Experiments}
\label{sec:experiment}
We conduct extensive experiments regarding the effectiveness of \textsf{\small CogSub2Q} and \textsf{\small CogSub$^m$2Q} using simple question to help complex question generation. Before that, let us first show the competitiveness of our base model \textsf{\small Cog2Q} in Section~\ref{sec:exp-T2S}.

Following previous work, we employ BLEU\footnote{Due to space limits, only BLEU-4 is shown in the tables below but we observe similar results on BLEU 1-3, which are included in the supplementary material.} \cite{Papineni2001BleuAM}, METEOR \cite{Banerjee2005METEORAA} and ROUGE-L \cite{Lin2004ROUGEAP} as automatic evaluation metrics, and discuss human evaluation results in Section~\ref{sec:exp-userstudy}. 
\add{These automatic metrics are evaluated on questions with placeholders to avoid the score inflation from long entity names.}

\input{tables_new/compare_encoder_less.tex}
\subsection{Base model comparison}
\label{sec:exp-T2S}
We compare our base model \textsf{\small Cog2Q} with some other existing models to show its competitiveness:
(1) The first baseline \textbf{SubQ} simply compare the closeness of a sub-question to a complex question. It shows the performance of naively copying every word from the sub-question. 
(2) The \textbf{Enc-Dec} baseline is adapted from the previous simple question generation work \cite{serban2016generating}, where the query graph is simplified as a bag of relation features that are built from $(s,p,o)$ triples the same way as \textsf{\small CoG2Q}, and the same decoder with relation attention and placeholder generation method is used. 
(3) The graph-to-sequence (\textbf{G2S}) model \cite{song-etal-2018-graph} is one of the state-of-the-art models from the AMR-to-text generation literature \cite{Flanigan2016GenerationFA, Konstas2017NeuralAS}.
We also adapt it to take as input the same set of features, and to use the exact same decoder as \textsf{\small CoG2Q}\nop{, but with a graph encoder versus the tree-LSTM encoder}.
% \fromH{may have a bit more details about the graph encoder??}
As shown in Table~\ref{tab:compare_encoder_less}, our base model \textsf{\small Cog2Q} outperforms all baselines, indicating the effectiveness of employing Tree-LSTM to aggregate the semantic information of a query graph from grounded entities to the question node.
It also indicates that sub-questions are not proximal to the target complex questions.
% All three neural encoder-decoder models are more effective than the naive method \textbf{SubQ}, which retrieves the ground-truth sub-question from WebQ and sacrifices the additional query graph relations. The \textbf{G2S} baseline outperforms \textbf{Enc-Dec}, showing that it is important to consider the structure of a complex query graph while encoding it.
% Our model \textsf{\small Cog2Q} further outperforms \textbf{G2S}, showing that it is more effective to treat KG query graphs as trees having the question nodes as roots, rather than unsorted graphs like those for AMR.

We also conduct an ablation study for \textsf{\small Cog2Q}\nop{, by removing the attention over relations, inverse predicate features, or the name features of the relations}, and the lower parts of Table~\ref{tab:compare_encoder_less} show the results.
We can see that the attention mechanism over relation triples is important, as it \add{creates a highway path over Tree-LSTM directly from relation encodings to the decoder.}
It also allows the decoder to focus on expressing different relations at different time steps.
\add{It is also helpful to learn the features vectors of a predicate when it appears in the inverse direction, which is another type of connection in CQG.} % Regarding the features representing a relation triple, \fromH{not very clear: we found that incorporating the learned embeddings of the inverse predicates helps the model learn to generate better questions, from examples containing relations in the inverse direction as well.}
In addition, encoding of the canonical names of the entity types and predicates contributes to the overall performance as well, because these names may contain words that have similar meanings to those appearing in the target questions.

% \input{tables_new/compare_using_multiple_subquestions_less.tex}
\subsection{Using sub-questions}
\label{sec:exp-TS2S}
The experiment results in the upper half of Table~\ref{tab:compare_using_subq} show that sub-questions from WebQ can help complex question generation. In particular, we observe: \fromH{I feel the analysis in this part is good, but we need to organize it more clearly and polish the verbiage.} 

(1) Straightforward data augmentation strategy (\textbf{+ data}) improves the performance of \textsf{\small Cog2Q} by incorporating the sub-questions as extra training samples.
Note that for fair comparison, we have used all the sub-questions (corresponding to not only training, but also validation and testing complex questions) as extra training samples.
% The reason is that when the model are explicitly taught to map the sub-queries to the sub-questions, it may also learn that the added relations should be mapped to the extra words in the complex questions but not in the sub-questions.

(2) More importantly, as discussed in Section~\ref{sec:incorp-subq}, we hypothesize that the data augmentation approach will be not as effective as using the sub-question in \textsf{\small CogSub2Q}, which can explicitly leverage the correspondence between the target complex question and its sub-questions.
The experiments verify this hypothesis.

(3) Very interestingly, we also discover that the sub-question correspondence information is essential to train the model successfully.
Specifically, we experiment with \textsf{\small CogSub2Q} in two different scenarios, one trained with randomly sampled pseudo sub-questions (marked with *) and the other one with actual sub-questions.
For both scenarios, only pseudo sub-questions are assumes at test time to generate a complex question, which is evaluated against multiple reference complex questions including the one corresponding to the randomly sampled pseudo sub-question.
For all experiments hereafter with such randomness, we show the average results of running the test data for 5 times in each scenario.
Table~\ref{tab:compare_using_multiple_subquestions} shows that \textsf{\small CogSub2Q} perform similarly to the data augmentation baseline when trained with pseudo sub-questions, but significantly better with actual sub-questions.
The reason for this is similar to why data augmentation is not optimal:
the sub-question to complex question mapping is less clearly established when the model learns from pseudo sub-questions instead of actual ones.
On the other hand, learning with sub-questions better exploits the intrinsic correspondence of the data, and it is easier for the model to learn with the actual sub-questions that often contain words appearing in the target complex questions.
\input{tables_new/compare_using_subq.tex}


\subsection{Using multiple pseudo sub-questions}
\label{sec:exp-TMS2S}
Assuming that sub-questions are not available, we now demonstrate whether pseudo sub-questions from SimpQ can help generate complex questions in the way sub-questions do in Section~\ref{sec:exp-TS2S}.
Table~\ref{tab:compare_using_pseudo} shows the results.
Different from previous, we only keep the complex questions with a relation appearing in SimpQ for fair comparison. \fromH{what do you mean? because of this, there is some difference between the two Cog2Q?}\fromJ{Yes, shall we mention it here?}
Similar to above, we report the results averaging 5 experiments.
\input{tables_new/compare_using_pseudo.tex}
% \fromH{Maybe we do not need to introduce the highest BLEU strategy in the previous training paragraph, and instead, we first state our observation on \textsf{\small CogSub2Q}(trained with rand.) and \textsf{\small CogSub$^m$2Q}(trained with rand.) and say "inspired by the previous discovery on association of sub-questions, we define the one with highest bleu as associated pseudo sub-questions and incorporate it into the set.." This way we can also make a connection between previous discovery and the design in this setting.}

% We experimented with both \textsf{\small CogSub2Q} and \textsf{\small CogSub$^m$2Q} under several settings.
First of all, it is consistent that data augmentation with simple questions helps the performance of \textsf{\small CoGSub2Q}.
We tested \textsf{\small CoGSub2Q} with randomly sampled pseudo sub-questions because real sub-questions are rare in SimpQ, and the results are similar to Section~\ref{sec:exp-TS2S} that it does not perform significantly better than data augmentation.
\add{The slight performance gain may come from that large number of pseudo sub-questions, which increases the robustness of the trained model.}
% There is no significant performance gain when randomly sampled simple questions are used for training and testing, or when using pseudo sub-questions with the highest BLEU for training but randomly sampled ones for testing.
% This behavior is different from WebQ, and we suspect the reason is because the SimpQ dataset has a much higher variance of the number of question per relation, and the simple questions are of different qualities.
% The inconsistency of training and testing, or exposure bias, even leads to that training with top BLEU simple questions getting lower metrics.
% We are able to notice significant performance gain only when using with pseudo-associated simple questions for both training and testing, but this a cheating scenario because it is impossible find out which simple question is associated with the to be generated complex question.
Finally, our proposed \textsf{\small CoGSub$^m$2Q} model taking as input multiple simple questions at once shows significant performance gain than \textsf{\small CoGSub2Q} with data augmentation \fromH{do you use all simpQ for augmentation or just those used in \textsf{\small CogSub$^m$2Q}?}\fromJ{only those used in our model}, proving that the model can simultaneous learn to predict higher association scores for more useful simple questions.

% \add{Would it be better if we have \textsf{\small CogSub$^m$2Q}(trained with rand)? We probably had it before, but I now think if \textsf{\small CogSub$^m$2Q}(trained with rand) can achieve similar performance to \textsf{\small CogSub$^m$2Q}(trained with assoc.), we can remove \textsf{\small CogSub$^m$2Q}(trained with assoc.) and \textsf{\small CogSub2Q}(trained with assoc.). Otherwise, we can show \textsf{\small CogSub2Q}(trained with rand.), \textsf{\small CogSub$^m$2Q}(trained with rand.), \textsf{\small CogSub$^m$2Q}(trained with assoc.), with the story/observation being that only using one or multiple randomly selected pseudo sub-questions are not as effective as including the one with highest BLEU, which is supposed to help select the best pseudo sub-question.}
% T/MS2S even outperforms the T/S2S baseline in the cheating scenarios, showing that the T/MS2S model learns better association scores than BLEU-based pseudo scores and benefits from using multiple simple questions at the same time.

\subsection{User study}
\label{sec:exp-userstudy}
To complement the automatic evaluations, we conduct a user study to compare the data augmentation method with our models that explicitly leverage (pseudo) sub-questions.
We ask \todo{??} human annotators who are all proficient English speakers to judge a generated question after seeing the corresponding query-graph and ground-truth complex questions.
We randomly sample 100 examples for the scenario with sub-questions and 100 examples for the scenario with pseudo sub-questions.
The human annotators are instructed to judge the correctness of a generated question, which is the percentage of constraints \add{relations?} that have been expressed correctly, and the naturalness of the overall generation with a score between 1 and 5.
Table~\ref{tab:user_study} shows the results.
In both scenarios, our method significantly outperforms the data augmentation counterpart in terms of correctness, indicating that our model can learn to leverage the (pseudo) sub-questions.
However, our methods do not achieve much higher naturalness scores.
This is probably because, despite directly copying a longer phrase from sub-questions may contribute to higher naturalness, the fusion of copied words and generated words is prone to unnatural connections.
\input{tables_new/user_study}





==> sections/intro_v2.tex <==
\section{Introduction}
\label{sec:intro}
%Automatic question generation is an important task that has gained a lot of attention recently, which aims to generate natural language questions from paragraphs \cite{Du2017LearningTA, Song2018LeveragingCI}, knowledge bases \cite{serban2016generating, elsahar2018zero} or images \cite{Patro2018MultimodalDN} etc.
%It can help generate datasets \cite{}, help computer to communicate with humans \cite{} and ???.
This work studies the problem of generating natural language questions from knowledge graph (KG) queries.  Automatic question generation is an important task that can help produce useful datasets \cite{} and enable machines communicate with humans \cite{} in natural language. Automatic KG based question generation has been widely studied recently, but with focus on \textit{simple} query that only have one relation. For example, \citet{serban2016generating} designed an encoder-decoder neural model to generate a question from a single KB relation triple (e.g., from ``\texttt{place\_of\_birth}" to ``\textit{Who is born in X?}"), and \citet{elsahar2018zero} further studies simple question generation in zero-shot settings to handle unseen predicates or entity types. However, existing work cannot generate questions from complex query graphs with multi-argument relations such as ``\textit{Who stared in the films directed by George Lucas?}" or composed logic such as ``\textit{What awards does the actress from Star Wars get?}".

% \nop{\fromH{to remove this paragraph: } In this work, we study the problem of generating natural language questions from knowledge graph (KG) queries, and specifically focus on generating complex questions.
% A KG is a directed graph where nodes are entities and edges are predicates depicting the relations between entities. 
% \add{For example, ({\tt fires\_creek}, {\tt contained\_by}, {\tt nantahala\_national\_forest}) states the fact that the creek is located within the forest.}
% Neural-based encoder-decoder methodologies have achieved superior results than template-based baselines, as studied in previous works about question generation from KG.
% \citet{serban2016generating} designed an encoder-decoder neural model to generate a question from a single KB relation. Their model is trained on SimpleQuestions \cite{weston2015towards}, a benchmark dataset curated for simple question answering, and contains a lot of training and testing examples sharing the same predicates or entity types, therefore making the task easy for question generation.
% This motivates \citet{elsahar2018zero} to further study simple question generation in zero-shot settings to explore the generalization performance to unseen predicates or entity types, and they discovered that using relevant text snippets from searching the web can help solve the zero-shot problem by adding a copying mechanism to the encoder-decoder model. \fromH{We leave the detailed discussion of the two work to related work.}
% However, the previous works only address simple question generation from KG, which is limited in use as they can not handle multi-argument relations such as \textit{What are the films directed by ???} or composed logic such as \textit{What ... ?}
% }

Therefore, here we investigate the problem of generating questions from \textit{complex} KG query graph, as shown in Figure \ref{fig:example}, and refer to it as \textit{complex question generation} (CQG). %which can be represented in graph structures that are called query graphs \cite{su2016generating}.
We generalize the methodology in previous work \cite{serban2016generating} to the complex question generation scenario, and design an encoder-decoder model named \textsf{\small Cog2Q}\footnote{which stands for \ul{co}mplex \ul{g}raph query to \ul{q}uestion.} with a tree-LSTM \cite{tai2015improved} encoder that can handle arbitrary query graphs, and an LSTM decoder with attention over individual relations.
However, it turns out that generating questions from complex query graphs is much more difficult than from simple ones, because all the relations need to be expressed in natural language coherently and in a logical order, and there is a lack of training instances that cover the large amount of different relation combinations. %a CQG model usually suffers from the training signal sparsity problem.
\nop{Therefore, more examples should be required to train a CQG system, otherwise it will suffer from the training signal sparsity problem.}
%We generalize the methodology of previous works to the complex question generation scenario, and design an encoder-decoder model with a tree-LSTM \cite{tai2015improved} encoder that can handle arbitrary query graphs, and a LSTM decoder with attention over query graph relations.
% Simple things should be simple, complex things should be possible\nop{quote Alan Kay}.
% Composing complex natural language utterances is difficult, but a human being is able to do this with many simple expressions in mind.
% This should be reflected in the automatic question generation system as well.

\begin{figure}
    \includegraphics[width=\linewidth]{figures/example.pdf}
    \centering
    \caption{An example of a complex query graph and question pair, with its sub-question and two pseudo sub-questions.}
    \label{fig:example}
\end{figure}

%\add{Observing the availability of simple questions such as XX and YY, we explore a new perspective of using \textit{sub-questions} of a complex query graph for question generation.}
\add{Intuitively, it is easier to build up a complex question from a simpler sub-question of it, e.g., by adding modifiers or clauses to the latter. 
Especially with KG, such sub-question to complex question associations can be clearly defined, if the query graph of the former is contained by the latter.}
Driven by this intuition, we develop a CQG model that can effectively leverage a sub-question of a complex query graph. To further consider the scenario where sub-questions are not available, we propose to use the simple questions in an existing dataset as surrogates and automatically learn the importance of each simple question for CQG.
% \add{Intuitively, it is easier to generate a complex question based on a simpler one, e.g., by adding modifiers or clauses to the latter. In fact, \citet{??} manually created a complex question $c$ by first expanding a simple query graph (and its question $s$) in XXX \cite{XX} using templates and then asking humans to paraphrase. Here $s$ is referred to as the \textit{sub-question} of $c$. Driven by this intuition, we develop a CQG model that can effectively leverage a sub-question of a complex query graph. To further consider the scenario where sub-questions are not available, we propose to use the simple questions in an existing dataset as surrogates and automatically learn the importance of each simple question for CQG.}
%Observing the availability of simple questions such as XX and YY, we explore a new perspective of using \textit{sub-questions} of a complex query graph for question generation
\nop{Generally speaking, we classify a sub-question to a complex question into two types: (1) strictly \emph{associated} and (2) \emph{pseudo-associated}.
The former means that the relations and entities asked in the sub-question exactly appears in the complex question, and it can be expanded into the complex question by adding more constraints.
The latter is more relaxed, and only requires the relation asked in the sub-question to be covered by the complex question, and they can be about different entities.}
% Hence, we focus on how to leverage existing sub-questions questions to help complex question generation.
% We study the following two cases:
% \begin{enumerate}[leftmargin=*]
%     \vspace{-0.3cm}
%     \item How to use \emph{associated} sub-questions to help generate complex questions.
%     \vspace{-0.3cm}
%     \item How to use \emph{unassociated} sub-questions when associated sub-questions are not available.
% \end{enumerate}

% Sub-question association is defined as follows: 
% \theoremstyle{definition}
% \begin{definition}{Sub-question Association.}
% A sub-question is associated to a complex question 
% \end{definition}

%There are a few challenges in utilizing the sub-questions.
A straightforward strategy to use simple question datasets is data augmentation, i.e., take them as additional instances to train a CQG model, but it does not fully exploit the information that one simple question is part of another complex one. 
Instead, we propose to fuse the above \textsf{\small Cog2Q} model with a seq2seq model \cite{see2017get} where the former encodes a complex query graph while the latter explicitly encodes a sub-question and the decoding process is enabled to copy words from the sub-question. We name this model as \textsf{\small CogSub2Q}.
%At test time, the model can leverage a randomly sampled sub-question to generate better complex questions.
% We fuse the base encoder-decoder model with a seq2seq model \cite{see2017get} that explicitly encodes a sub-question and jointly contributes to the decoding process, and find this approach to be more effective than plainly incorporate the sub-questions as additional training examples.
% Interestingly, however, we also discover that the human composition association between sub-questions and complex questions is essential to training such a model effectively.
% This is because the questions can occur in many different paraphrases, and it is difficult to train the model to compose a complex question from a paraphrase of its sub-question, but with which it shares few lexicons in common.
% On the other hand, when such associations are available for training, the model during testing can leverage a randomly sampled sub-question to generate better complex questions.

On the other hand, in practice, sub-questions associated with a given complex query graph may not be available. In such scenarios, given a complex query graph $G$, we use simple questions that correspond to a subset of predicts in $G$ as its \textit{pseudo sub-questions}.
\add{We assume that pseudo sub-questions with the highest BLEU score with the to-be-generated complex question can be treated as real sub-questions.
Interestingly, however, we discover that such pseudo sub-questions do not improve the performance as much as real sub-questions do in \textsf{\small CogSub2Q} before, compared with random sampling.
}
\nop{Interestingly, we discover that treating all pseudo sub-questions equally and randomly sampling one to use \textsf{\small CogSub2Q} as before will not work. % We discover that the association between sub-questions and complex questions is essential to effectively training the model.
We hypothesize that this is because questions can have many different paraphrases, and it is difficult to train the model if a sub-question has few tokens in common with the to-be-generated complex question.
% To verify this hypothesis, we choose the pseudo sub-question with the highest BLEU score with the to-be-generated complex question to train and test the model, which shows better performance than randomly sampling a pseudo sub-question. 
% In practice, however, this strategy is not applicable, as it requires to know the to-be-generated complex question at test time.
}
To solve this problem, we propose \add{to let the model learn which pseudo sub-questions maybe more helpful and design} a new model \textsf{\small CogSub$^m$2Q} by further extending \textsf{\small CogSub2Q} to take in multiple pseudo sub-questions. \textsf{\small CogSub$^m$2Q}  simultaneously learns to predict an association score for each pseudo sub-question and composes the complex question based on them according to their association levels.
Experimental results on the ComplexWebQuestions \cite{talmor2018web} datasets show that \add{\textsf{\small CogSub2Q} and }\textsf{\small CogSub$^m$2Q} can effectively utilize \add{sub-questions and }multiple pseudo sub-questions to generate better complex questions.
% However, associated simple questions may not always be available.
% So, we further study whether we can leverage the large amount of unassociated simple questions for complex questions generation.
% Same as before, training without considering association is not successful, but the key observation is that complex question generation can benefit from pseudo associated simple questions, with word-matching as a proxy for association.
% However, the model still suffers at test time from the large amount of simple questions with different association qualities.
% Therefore, we propose to solve the problem by extending the proposed model to take in multiple sub-questions.
% It simultaneously learns to predict an association score for the sub-questions as well as to compose the complex question based on them according to their association levels.
% Experiments results show that this model can generate better complex questions by leveraging unassociated simple questions.

% In summary, our contributions are:
% \begin{itemize}[leftmargin=*]
% \vspace{-5mm}
% \item To the best of our knowledge, we are the first to study the problem of complex question generation from knowledge graphs. We follow the methodologies of previous works and design an encoder-decoder model suitable for the task.
% \vspace{-5mm}
% \item We find that it is effective to explicitly leverage sub-questions for complex question generation through a specific sub-question encoder. We also find that the simple to complex question association is essential to train such a model.
% \vspace{-5mm}
% \item We further explore the scenario where the associated sub-questions are not available, and propose to leverage the easily available simple questions. We extend the model to work with multiple simple question paraphrases, and allow it to simultaneously learn which one to emphasis on from pseudo simple to complex associations defined by word matching.
% \end{itemize}

% \todo{List out challenges that we have, the questions that we want to answer, let the base model description after the two scenarios of using sub-questions (hard to explain the following model)??}

==> sections/intro_v3.tex <==
\section{Introduction}
\label{sec:intro}
\nop{This work studies the problem of generating natural language questions from knowledge graph (KG) queries.}
Automatic question generation is an important task that can help produce useful datasets \cite{} and enable machines communicate with humans \cite{} in natural language. Automatic KG based question generation has been widely studied recently, but with focus on \textit{simple} queries that only contains one relation. For example, \citet{serban2016generating} designed an encoder-decoder neural model to generate a question from a single KB relation triple, e.g., from \nop{(\texttt{\small{Padm\'e Amidala}}, \texttt{\small{children}}, \texttt{\small{Leia Organa}})}(\texttt{\small{Leia Organa}}, \texttt{\small{parent}}, \texttt{\small{Padm\'e Amidala}}) to ``\textit{Who is Princess Leia's mothter?}". \citet{elsahar2018zero} further studies simple question generation in zero-shot settings to handle unseen predicates or entity types by incorporating external context information. 
However, existing work cannot generate questions from complex query graphs with multi-argument relations or composed logic.

\begin{figure}
    \includegraphics[width=\linewidth]{figures/example.pdf}
    \centering
    \caption{An example of a complex query graph and question pair, with its sub-question and two pseudo sub-questions.}
    \label{fig:example}
\end{figure}

Motivated by the above limitation, this work makes one of the first efforts toward generating questions from \textit{complex} KG query graphs, as shown in Figure \ref{fig:example}, and refer to this problem as \textit{complex question generation} (CQG). 
We first design an encoder-decoder model named \textsf{\small CoG2Q}\footnote{which stands for \ul{Co}mplex \ul{G}raph query to \ul{Q}uestion.} with a tree-LSTM \cite{tai2015improved} encoder that can handle arbitrary query graphs, and an LSTM decoder with attention over individual relations.
However, it turns out that generating questions from complex query graphs is much more difficult than from simple ones, because all the relations need to be expressed in natural language correctly and coherently. Unfortunately, there is a lack of training instances that cover the exponentially growing amount of different relation combinations.

A straight-forward strategy of using simple question datasets to improve the CQG performance is data augmentation\fromJ{need citation?}, i.e., using the simple questions as additional training instances.
This strategy is well suited for the one-size-fit-all \textsf{\small CoG2Q} model, which handles simple and complex question generation indiscriminately.
However, this only establish \emph{model-level} connection between the simple and complex training instances through jointly trained model parameters, and does not fully exploit the intrinsic connections between simple and complex instances within the datasets.
\nop{REORGANIZE: Not surprisingly, existing simple question datasets can be used to improve the CQG performances.
However, the one-size-fit-all characteristic of the above \textsf{\small CoG2Q} model leads to a problem: since the model handles simple and complex question generation indiscriminately, a simple question datasets can only be used for data augmentation, i.e. as additional instances for training.}

To remedy this, we explore how to leverage finer grained connections, and specifically look into two scenarios: leveraging sub-questions and pseudo sub-questions for CQG.
A sub-question of a complex question can be clear defined with KG, if the query graph of the former is contained in the latter.
Pseudo sub-questions are similar to sub-questions, but with the condition relaxed that it may be asking about different entities, which makes them much easier available. 
The \emph{instance-level} connections with (pseudo) sub-questions may be useful, because intuitively it is easier to generate a complex question while accessing the sub-questions of its own.

We prove this idea by developing a CQG model that explicitly encode a sub-question of the to-be-generated complex question and use the encoded results in the decoding process as well. We name this model as \textsf{\small CoGSub2Q}.
Our empirical results show that the sub-question to question associations are important to train the model effectively.
And in the scenario where sub-questions are not be readily available, we use randomly sampled pseudo sub-questions from an existing dataset as surrogates.
% \nop{REORGANIZE:
% And in the scenario where sub-questions are not be readily available, we use randomly sampled pseudo sub-questions from an existing dataset as surrogates but find it achieves sub-optimal performances.
% The reason is that the sub-question and question associations are important to train the model successfully, as we empirically discovered with sub-questions.
To compensate for the lack of actual sub-questions associations, we propose to further extend \textsf{\small CoGSub2Q} into \textsf{\small CoGSub$^m$2Q}, which takes in multiple pseudo sub-questions and simultaneously learns to predict an association score for each of them. 
The scores are then used to aggregate the pseudo sub-questions to help generate the final complex question.
Experimental results on the ComplexWebQuestions \cite{talmor2018web} datasets show that \textsf{\small CoGSub2Q} and \textsf{\small CoGSub$^m$2Q} can effectively utilize sub-questions and multiple pseudo sub-questions to generate better complex questions.


==> sections/intro_v4.tex <==
\section{Introduction}
\label{sec:intro}
Automatic question generation is an important task that can help produce useful datasets \cite{serban2016generating,Jain2017CreativityGD,Guo2018QuestionGF} and facilitate\nop{enrich} human-machine communication through natural language \cite{Wang2018LearningTA,Gur2018DialSQLDB}. 
Knowledge graph (KG) has been a popular data source for question generation, but with a focus on \textit{simple} queries each containing only one relation. For example, \citet{serban2016generating} design an encoder-decoder neural model to generate a question from a single KB relation triple, e.g., from (\texttt{\small{Padm\'e Amidala}}, \texttt{\small{children}}, \texttt{\small{Leia Organa}})\nop{(\texttt{\small{Leia Organa}}, \texttt{\small{parent}}, \texttt{\small{Padm\'e Amidala}})} to ``\textit{Who is Queen Amidala's child?}". 
\citet{elsahar2018zero} further study simple question generation in zero-shot settings to handle unseen predicates or entity types by incorporating external context information. 
However, existing work cannot generate questions from complex query graphs with multi-argument relations or composite logic.
\begin{figure}
    \includegraphics[width=\linewidth]{figures/example.pdf}
    \centering
    % \vspace{-0.7cm}
    \caption{An example of a complex query graph and question pair, with its \textit{sub-question} and two \textit{pseudo sub-questions} (See Definition~\ref{def:subq} and \ref{def:pseudo-subq} in Section~\ref{sec:preliminary}).}
    % \vspace{-0.4cm}
    \label{fig:example}
\end{figure}

Therefore, we are motivated to make one of the first efforts toward \textit{complex question generation} (CQG): given a query graph with more than one relation, output a complex question that has the same meaning, as exemplified in Figure~\ref{fig:example}.
It is much more challenging to generate questions from complex query graphs than simple ones, because all the relations need to be expressed in natural language correctly and coherently. 
Unfortunately, there is a lack of training instances that can cover the exponentially growing amount of different relation combinations.
Consequently, it is desirable to effectively leverage existing simple questions for CQG.
In particular, we examine two separate scenarios, with either \emph{sub-questions} of the to-be-generated complex question, or with only distantly related \emph{pseudo sub-questions} that are about other entities (when sub-questions are unavailable).
% We will formally define (pseudo) sub-questions in Section~\ref{sec:preliminary}, but Figure~\ref{fig:example} shows the example of one sub-question and two pseudo sub-questions.
% We observe that sub-questions are more similar to the target complex question, while the pseudo sub-question can be more easier to acquire.
% In the first scenario, we assume the availability of sub-questions of the to-be-generated complex question for training, such as the one in Figure~\ref{}.
% In the second scenario, we restrict the assumption with only pseudo sub-questions, which are distantly related to the complex question through a shared predicate (e.g. \texttt{\small parent}).

We first design a base encoder-decoder model for CQG named \textsf{\small CoG2Q}\footnote{which stands for \ul{Co}mplex query \ul{G}raph to \ul{Q}uestion.}.
It has a tree-LSTM \cite{tai2015improved} encoder that can handle arbitrary query graphs, and an LSTM \cite{Hochreiter1997LongSM} decoder with attention over individual relations.
A straightforward strategy to improve the CQG performance with simple questions is data augmentation, i.e., using them as additional training instances.
This strategy is well suited for the one-size-fits-all \textsf{\small CoG2Q} model, which handles simple and complex question generation indiscriminately.
However, it only establishes \emph{model-level} connections between all the simple and all the complex questions through jointly fitted model parameters, which may be sub-optimal due to the underexploitation of the specific correspondence between a complex question and its (pseudo) sub-questions.
% \nop{REORGANIZE: Not surprisingly, existing simple question datasets can be used to improve the CQG performances.
% However, the one-size-fit-all characteristic of the above \textsf{\small CoG2Q} model leads to a problem: since the model handles simple and complex question generation indiscriminately, a simple question datasets can only be used for data augmentation, i.e. as additional instances for training.}

In contrast\nop{On the contrary}, our proposed extension models \textsf{\small CoGSub2Q} and \textsf{\small CoGSub$^m$2Q} can exploit \emph{instance-level} connections between simple and complex questions for CQG.
% A sub-question of a complex question can be clear defined with KG, if the query graph of the former is contained in the latter.
% Pseudo sub-questions are similar to sub-questions, but with the condition relaxed that it may be asking about different entities, which makes them much easier available. 
% The \emph{instance-level} connections with (pseudo) sub-questions may be useful, because intuitively it is easier to generate a complex question while accessing the sub-questions of its own.
\textsf{\small CoGSub2Q} is used in the first scenario, which additionally encodes a sub-question and explicitly copies words from it while generating the target complex question.
Empirical results show that this model can be trained effectively with the sub-question associated to the complex question.
\textsf{\small CoGSub$^m$2Q} is designed for the second scenario where pseudo sub-questions from an existing dataset are used as surrogates for sub-questions.
% \nop{REORGANIZE:
% And in the scenario where sub-questions are not be readily available, we use randomly sampled pseudo sub-questions from an existing dataset as surrogates but find it achieves sub-optimal performances.
% The reason is that the sub-question and question associations are important to train the model successfully, as we empirically discovered with sub-questions.
To compensate for the lack of actual sub-questions, \textsf{\small CoGSub$^m$2Q} simultaneously takes as input multiple pseudo sub-questions, which are scored and aggregated to help generate the final complex question.
Experimental results on the ComplexWebQuestions \cite{talmor2018web} dataset show that \textsf{\small CoGSub2Q} and \textsf{\small CoGSub$^m$2Q} can more effectively utilize sub-questions and multiple pseudo sub-questions than straightforward data augmentation, and generate better complex questions.\nop{can utilize sub-questions and multiple pseudo sub-questions to generate better complex questions, which is more effective than straightforward data augmentation}



==> sections/introduction.tex <==
\section{Introduction}
Automatic question generation is an important task that has gained a lot of attention recently, which aims to generate natural language questions from paragraphs \cite{Du2017LearningTA, Song2018LeveragingCI}, knowledge bases \cite{serban2016generating, elsahar2018zero} or images \cite{Patro2018MultimodalDN} etc.
It can help generate datasets \cite{}, help computer to communicate with humans \cite{} and ???.

In this work, we study the problem of generating natural language questions from knowledge graph (KG) queries, and specifically focus on generating complex questions.
A KG is a directed graph where nodes are entities and edges are predicates depicting the relations between entities. 
\add{For example, ({\tt fires\_creek}, {\tt contained\_by}, {\tt nantahala\_national\_forest}) states the fact that the creek is located within the forest.}
Neural-based encoder-decoder methodologies have achieved superior results than template-based baselines, as studied in previous works about question generation from KG.
\citet{serban2016generating} designed an encoder-decoder neural model to generate a question from a single KB relation. Their model is trained on SimpleQuestions \cite{weston2015towards}, a benchmark dataset curated for simple question answering, and contains a lot of training and testing examples sharing the same predicates or entity types, therefore making the task easy for question generation.
This motivates \citet{elsahar2018zero} to further study simple question generation in zero-shot settings to explore the generalization performance to unseen predicates or entity types, and they discovered that using relevant text snippets from searching the web can help solve the zero-shot problem by adding a copying mechanism to the encoder-decoder model.
However, the previous works only address simple question generation from KG, which is limited in use as they can not handle multi-argument relations such as \textit{What are the films directed by ???} or composed logic such as \textit{What ... ?}

In this work, we explore the problem of generating question from complex KG queries, which can be represented in graph structures that are called query graphs \cite{su2016generating}.
We generalize the methodology of previous works to the complex question generation scenario, and design an encoder-decoder model with a tree-LSTM \cite{tai2015improved} encoder that can handle arbitrary query graphs, and a LSTM decoder with attention over query graph relations.
Generating complex natural language questions is much more difficult than from simple ones, because all the relations need to be expressed coherently and connected by the correct logic.
Therefore, more examples should be required to train a CQG system, otherwise it will suffer from the training signal sparsity problem. 
% Simple things should be simple, complex things should be possible\nop{quote Alan Kay}.
% Composing complex natural language utterances is difficult, but a human being is able to do this with many simple expressions in mind.
% This should be reflected in the automatic question generation system as well.
Generally speaking, we classify a sub-question to a complex question into two types: (1) strictly \emph{associated} and (2) \emph{pseudo-associated}.
The former means that the relations and entities asked in the sub-question exactly appears in the complex question, and it can be expanded into the complex question by adding more constraints.
The latter is more relaxed, and only requires the relation asked in the sub-question to be covered by the complex question, and they can be about different entities.
% Hence, we focus on how to leverage existing sub-questions questions to help complex question generation.
% We study the following two cases:
% \begin{enumerate}[leftmargin=*]
%     \vspace{-0.3cm}
%     \item How to use \emph{associated} sub-questions to help generate complex questions.
%     \vspace{-0.3cm}
%     \item How to use \emph{unassociated} sub-questions when associated sub-questions are not available.
% \end{enumerate}

% Sub-question association is defined as follows: 
% \theoremstyle{definition}
% \begin{definition}{Sub-question Association.}
% A sub-question is associated to a complex question 
% \end{definition}

There are a few challenges in utilizing the sub-questions.
First, using the associated sub-questions as augmented training samples does not fully exploit the association.
Instead, we propose to fuse the base encoder-decoder model with a seq2seq model \cite{see2017get} that explicitly encodes a sub-question and jointly contributes to the decoding process.
Interestingly, we discover that the association between sub-questions and complex questions is essential to training such a model effectively.
This is because the questions can occur in many different paraphrases, and it is difficult to train the model to compose a complex question from a paraphrase of its sub-question, but with which it shares few lexicons in common.
At test time, the model can leverage a randomly sampled sub-question to generate better complex questions than using data augmentation.
% We fuse the base encoder-decoder model with a seq2seq model \cite{see2017get} that explicitly encodes a sub-question and jointly contributes to the decoding process, and find this approach to be more effective than plainly incorporate the sub-questions as additional training examples.
% Interestingly, however, we also discover that the human composition association between sub-questions and complex questions is essential to training such a model effectively.
% This is because the questions can occur in many different paraphrases, and it is difficult to train the model to compose a complex question from a paraphrase of its sub-question, but with which it shares few lexicons in common.
% On the other hand, when such associations are available for training, the model during testing can leverage a randomly sampled sub-question to generate better complex questions.

Second, when associated sub-questions may not always be available.
In such cases, we study whether we can leverage the large amount of pseudo-associated simple questions for complex questions generation.
However, qualities of the pseudo-associated sub-questions have high variance, so treating them as equally associated and using the same strategy as before fails.
We discovered that using word-overlapping as a proxy association score makes the model work, but this requires unrealistically to known the more associated sub-question at test time.
To solve this problem, we propose to extend the previous model to take in multiple sub-questions.
It simultaneously learns to predict an association score for the sub-questions as well as to compose the complex question based on them according to their association levels.
Experiments results show that this model can generate better complex questions by leveraging unassociated simple questions.
% However, associated simple questions may not always be available.
% So, we further study whether we can leverage the large amount of unassociated simple questions for complex questions generation.
% Same as before, training without considering association is not successful, but the key observation is that complex question generation can benefit from pseudo associated simple questions, with word-matching as a proxy for association.
% However, the model still suffers at test time from the large amount of simple questions with different association qualities.
% Therefore, we propose to solve the problem by extending the proposed model to take in multiple sub-questions.
% It simultaneously learns to predict an association score for the sub-questions as well as to compose the complex question based on them according to their association levels.
% Experiments results show that this model can generate better complex questions by leveraging unassociated simple questions.

% In summary, our contributions are:
% \begin{itemize}[leftmargin=*]
% \vspace{-5mm}
% \item To the best of our knowledge, we are the first to study the problem of complex question generation from knowledge graphs. We follow the methodologies of previous works and design an encoder-decoder model suitable for the task.
% \vspace{-5mm}
% \item We find that it is effective to explicitly leverage sub-questions for complex question generation through a specific sub-question encoder. We also find that the simple to complex question association is essential to train such a model.
% \vspace{-5mm}
% \item We further explore the scenario where the associated sub-questions are not available, and propose to leverage the easily available simple questions. We extend the model to work with multiple simple question paraphrases, and allow it to simultaneously learn which one to emphasis on from pseudo simple to complex associations defined by word matching.
% \end{itemize}

% \todo{List out challenges that we have, the questions that we want to answer, let the base model description after the two scenarios of using sub-questions (hard to explain the following model)??}

==> sections/model_base.tex <==
\section{Tree2Seq as Base Model for CQG}
\label{sec:T2S}

We follow previous single-relation question generation work to use a encoder-decoder framework, but adapt the model for complex question generation.
Specifically, the model consists of a Tree-LSTM encoder \cite{tai2015improved} and LSTM decoder \cite{hochreiter1997long} and is therefore named Tree2Seq, or \textbf{T2S} for short.
% We also compared this model with some variants: treating relations as an unordered sequence and using Graph network for the encoder.

\subsection{Encoder}
\noindent\textbf{Encode relations.}
A relation $r$ is a tuple $(s, p, o)$.
First, node $s$ and $o$ are mapped to feature vectors $f^{(s)}$ and $f^{(o)}$, each being the concatenation of two vectors: one determined by its specific entity type\footnote{Freebase predicates determined the entity type of its subjects and objects.} and the other determined by whether it is an answer node, an internal node or a terminal node.
% The second vector partially preserve the structural information.
We do not use the vector representations of specific KG entities as in previous work for two reasons.
First, use the node type information as input should be enough because the task is to generate placeholders rather than entity names.
Second, our approach do not require all the entities to actually appear in the KG as previous work do, allowing it to be more generally applicable (i.e. it can generate questions for KG expansion).
For a predicate $p$ in KG, there is usually a corresponding inverse relation $\neg p$.
We concatenate the vector representations of both $p$ and $\neg p$ as the predicate feature $f^{(p)}$, so that the model can learn the relation between a question and its inverse.

We also use the names of entity types and predicates \footnote{Retained by Freebase predicate \tt{type.object.name}} towards the encoding of a relation.
Specifically, the canonical names of $s$, $p$ and $o$ are joined into a token sequence by delimiter $\langle\mathrm{d}\rangle$: $n^{(r)} \text{$=$} [n^{(s)}_1 ... n^{(s)}_{L^{(s)}} \langle\mathrm{d}\rangle n^{(p)}_1 ... n^{(p)}_{L^{(p)}} \langle\mathrm{d}\rangle n^{(o)}_1 ... n^{(o)}_{L^{(o)}}]$.
It is then pass through an LSTM network and the final hidden state is $h^\text{(N)}_{L}$, where $L\text{$=$}L^{(s)}\text{$+$}L^{(p)}\text{$+$}L^{(o)}\text{$+$}2$ is the length of $n^{(r)}$.
Finally, all the above feature vectors are concatenated and passed through a fully connected neural layer to be the relation encoding vector $e^{(r)}$:
\begin{align}
    &[h^\text{(N)}_0 ... h^\text{(N)}_{L}] = \text{LSTM}^\text{(N)}(n^{(r)}) ,\\
    &e^{(r)} = \mathrm{tanh}(W[f^{(s)}, f^{(p)}, f^{(o)}, h^\text{(N)}_{L}] + b) .
\end{align}

\noindent\textbf{Encode query graph.}
The relations encoding vectors are used in a tree-LSTM network to generate the encoding of the entire query graph and preserve its structural information.
Due to space limits, we do not introduce the detailed architecture of the tree-LSTM cell and refer readers to \citet{tai2015improved} for details.
We treat the answer node as root, and use topological sort to break any circles in the query graph to make it into a tree (duplicating nodes if necessary).
Because the children nodes in the query tree are unordered and their number is unfixed, the child-sum version of tree-LSTM is used.
Generally, a tree-LSTM cell works as follows at each time step, computing the hidden states of a node after all its children nodes:
% In sum, at each time step, a tree-LSTM cell calculates the hidden state of a node with an input vector $r^\text{enc}_j$ that is the encoding of the relation corresponds to the edge connecting the node to its parent, and the hidden states of all its children $C_j$. Formally:
\begin{equation}
    \label{eq:tree-lstm}
    h^\text{(T)}_j = \mathrm{TreeLSTMCell}(e^{(r)}_j, \{h^\text{(T)}_k\}_{k\in C_j}) .
\end{equation}
% \begin{align}
%     h^{\sim}_j &= \textstyle\sum_{k\in C(j)}h_k ,\\
%     i_j &= \sigma(W^{(i)}[enc(r_j), h^{\sim}_j]+b^{(i)}) ,\\
%     f_{jk} &= \sigma(W^{(f)}[enc(r_j), h^{\sim}_j]+b^{(f)}) ,\\
%     o_j &= \sigma(W^{(o)}[enc(r_j), h_k]+b^{(o)}) ,\\
%     u_j &= tanh(W^{(u)}[enc(r_j), h^{\sim}_j]+b^{(u)}) ,\\
%     c_j &= i_j \odot u_j + \textstyle\sum_{k\in C(j)} f_{jk} \odot c_k ,\\
%     h_j &= o-j \odot tanh(c_j) .
% \end{align}
Specifically for node $o_j$, we use the encoding $e^{(r)}_j$ corresponding to $r_j\text{$=$}(s_j, r_j, o_j)$ as input; and $C_j$ represents the set of all children nodes of $o_j$.
% Note that this relation corresponds to the edge that connects $o_j$ corresponds to its parent.
Note that the leaf (grounded) nodes and the root (answer) nodes are the special cases.
For leaf nodes, a zero vector is used as the hidden state for their nonexistent ``children''; for root nodes, a dummy relation encoding $e^{(r)}_\text{dummy}$ is used as the input. 

\subsection{Decoder}
\noindent\textbf{LSTM decoder with attention over relations.}
We use an LSTM decoder to generate the question tokens.
Its hidden states are initialized by that of the tree-LSTM.
An attention \cite{bahdanau2014neural} and coverage \cite{see2017get} mechanism over the encoding of relations is also employed to encouraging the decoder to generate tokens covering all of them. 
At time step $t$:
\begin{align}
    h_t &= \mathrm{LSTMCell}^{(d)}(x_{t-1}, h_{t-1}) ,\\
    % e_{tj} &= w^{T} \mathrm{tanh}(W[h_t, r^\mathrm{enc}_j, c_{tj}]+b) ,\\
    % a_{tj} &= \mathrm{exp}(e_{tj}) / \textstyle\sum_{k} \mathrm{exp}(e_{tk}) ,\\
    c_{tj} &= \textstyle\sum_{t'=0}^{t-1}a_{t'j}, \\
    a_{tj} &\propto w^{T} \mathrm{tanh}(W[h_t, e^{(r)}_j, c_{tj}]+b) ,\\
    r^*_t &= \textstyle\sum_{j} a_{tj} e^{(r)}_j ,
\end{align}
where $h_{t-1}$ is the previous hidden state of the decoder LSTM; $x_{t-1}$ is the word embedding of the previous generated token; $a_{tj}$($c_{tj}$) is the attention(coverage) on relation $r_j$ at timestep $t$; and $r^*_t$ is the context vector.
Then, the probability distribution of generating words from the vocabulary is 
\begin{equation}
\label{eq:p_vocab}
    P_\text{vocab} = \mathrm{softmax}(W[h_t, r^*_t] + b).
\end{equation}

\noindent\textbf{Placeholder generation.}
As discussed earlier, we use placeholders to represent entities. 
Placeholder can not be generated in the same way as vocabulary words, because they represents different entities in different query graphs and do not have a global meaning.
We design a novel placeholder generation method by reusing the attention over relations, noticing that each relation connects to at most one grounded entity.
Specifically, $p_\text{ph}\in[0,1]$ controls the probability of generating a placeholder $P(w | w \text{$=$}\text{ph}(o_j))$ for $o_j$ versus of from the vocabulary$P(w | w\text{$\in$}\text{vocab})$:
\begin{align}
    &p_\text{ph} = \sigma(W[x_t, h_t, r^*_t] + b) , \label{eq:p_ph}\\
    &P(w | w\text{$\in$}\text{vocab}) = (1 - p_\text{ph}) P_\text{vocab}(w) , \label{eq:prob_vocab} \\
    &P(w | w\text{$=$}\text{ph}(o_j)) = p_\text{ph} \alpha'_{tj}. \label{eq:prob_placeholder}
\end{align}
Here, $\alpha_{ij}'$ slightly differs from the the attention $\alpha_{ij}$ in that it is the softmax of $e_{ij}$ after those relations not attached to a terminal entity are set to zero.

\subsection{Training}
\label{sec:t2s_train}
The model can be trained with Maximum Likelihood Estimation to optimize the probability of generating the ground truth token $w^*$, either from the vocabulary (Eq.\ref{eq:prob_vocab}) or is a placeholder (Eq.\ref{eq:prob_placeholder}), at each time step.
We also add a coverage loss $\mathcal{L}_\text{COV}$ to  encourage attending over all the relations and a L2 regularizer to prevent overfitting:
\begin{align}
    % &\mathcal{L}_\mathrm{MSE} = \begin{cases}
    %     -log(P_\text{vocab}(w^*)),&\text{ $w^*\text{$\in$}\text{vocab}$} \\
    %     -log(P_\text{ph}(w^*))),&\text{ $w^*$=$\text{ph}(o_j)$}
    %     \end{cases} ,\\
    &\mathcal{L}_\text{MSE} = -log(P(w^*)), \\
    &\mathcal{L}_\text{COV} = \textstyle\sum_{j} \text{min}(a_{tj}, c_{tj}) ,\\
    &\mathcal{L} = \mathcal{L}_\text{MSE} + \lambda_1 \mathcal{L}_\text{COV} + \lambda_1 L2 .
\end{align}





==> sections/model_base_v1.tex <==

\section{\textsf{\small CoG2Q}: Base Model for CQG}
\label{T2S}

Our base model for CQG, named \textsf{\small CoG2Q} (\ul{Co}mplex \ul{G}raph to \ul{Q}uestion), takes a query graph as input and outputs a natural language question using the popular encoder-decoder paradigm. The encoder in \textsf{\small CoG2Q} is adapted from the Tree-LTSM encoder \cite{tai2015improved}  with our unique way to represent relation triples, while the decoder in \textsf{\small CoG2Q} is built on top of an LSTM decoder \cite{hochreiter1997long} with a novel strategy to generate entity placeholders as well as an attention mechanism over multiple relation triples.
The black components in Figure~\ref{fig:model} shows an overview of \textsf{\small CoG2Q}.

\subsection{Encoder}
\noindent\textbf{Tree-LSTM for encoding a query graph.} Let us assume each relation triple has been encoded as a vector for now. The tree-LSTM network \cite{tai2015improved} will use them to generate the encoding of the entire query graph and preserve its structural information. We treat the answer node as root, and use topological sort to break any circles in the query graph to make it into a tree (duplicating nodes if necessary). Generally, a tree-LSTM aggregates information from leaf nodes to the root, and the hidden states of a node incorporates that of all its child nodes. Specifically in our case:
% \fromH{Move this to supplementary material or footnote/exp if there is space: Because the children nodes in the query tree are unordered and their number is unfixed, the child-sum version of tree-LSTM is used.}

% In sum, at each time step, a tree-LSTM cell calculates the hidden state of a node with an input vector $r^\text{enc}_j$ that is the encoding of the relation corresponds to the edge connecting the node to its parent, and the hidden states of all its children $C_j$. Formally:
\begin{equation}
    \label{eq:tree-lstm}
    h^\text{(T)}_j = \mathrm{TreeLSTMCell}(e^{(r)}_j, \{h^\text{(T)}_k\}_{k\in C_j}) ,
\end{equation}
% \begin{align}
%     h^{\sim}_j &= \textstyle\sum_{k\in C(j)}h_k ,\\
%     i_j &= \sigma(W^{(i)}[enc(r_j), h^{\sim}_j]+b^{(i)}) ,\\
%     f_{jk} &= \sigma(W^{(f)}[enc(r_j), h^{\sim}_j]+b^{(f)}) ,\\
%     o_j &= \sigma(W^{(o)}[enc(r_j), h_k]+b^{(o)}) ,\\
%     u_j &= tanh(W^{(u)}[enc(r_j), h^{\sim}_j]+b^{(u)}) ,\\
%     c_j &= i_j \odot u_j + \textstyle\sum_{k\in C(j)} f_{jk} \odot c_k ,\\
%     h_j &= o-j \odot tanh(c_j) .
% \end{align}
here $e^{(r)}_j$ represents the encoding of relation triple $r_j\text{$=$}(s_j, p_j, o_j)$; $h^\text{(T)}_j$ is the hidden states of $o_j$; and $C_j$ is the set of all child nodes of $o_j$.
Due to space limits, we refer readers to the supplementary material\nop{\citet{tai2015improved}} for more details about the Tree-LSTM architecture and the special handling of leaf and root nodes.
% \fromH{do not forget to include this, or maybe refer the readers to the child-sum part in the original paper.}
% Note that this relation corresponds to the edge that connects $o_j$ corresponds to its parent.
% \fromH{More this to supplementary material: Note that the leaf (grounded) nodes and the root (answer) nodes are the special cases.
% For leaf nodes, a zero vector is used as the hidden state for their nonexistent ``children''; for root nodes, a dummy relation encoding $e^{(r)}_\text{dummy}$ is used as the input. }

\input{tables_new/relation_features.tex}
\noindent\textbf{Encode relations.}
Now we clarify how we encode a relation triple $r$=$(s, p, o)$. 
First, node $s$ and $o$ are mapped to feature vectors $f^{(s)}$ and $f^{(o)}$, each being the concatenation of two vectors: one determined by its entity type\footnote{Each Freebase predicate has a pairs of designated type signatures for its connected entities \cite{berant2013semantic}.} and the other determined by whether it is a question node, an internal variable node or a terminal node.
% The second vector partially preserve the structural information.
We do not use the vector representations of specific KG entities as in previous work for two reasons:
First, use the node type information as input should be enough because the task is to generate placeholders rather than entity names.
Second, our approach does not require all the entities to \fromH{have pre-learnt embeddings at test time?} \add{This is not accurate, right? as if not in KG, then why you have the query graph?: actually appear in the KG} as previous work do, allowing it to be more generally applicable (i.e. \add{not sure: it can generate questions for KG expansion}).
For a predicate $p$ in KG, there is usually a corresponding inverse relation $\hat{}p$.
We concatenate the vector representations of both $p$ and $\hat{}p$ as the predicate feature $f^{(p)}$, so that the model can learn the relation between a question and its inverse.

We also use the names of entity types and predicates\footnote{Retained by Freebase predicate \tt{type.object.name}} for encoding a relation triple.
Specifically, the canonical names of $s$, $p$ and $o$ are concatenated into a token sequence by delimiter $\langle\mathrm{d}\rangle$: $n^{(r)} \text{$=$} [n^{(s)}_1 ... n^{(s)}_{L^{(s)}} \langle\mathrm{d}\rangle n^{(p)}_1 ... n^{(p)}_{L^{(p)}} \langle\mathrm{d}\rangle n^{(o)}_1 ... n^{(o)}_{L^{(o)}}]$.
It is then passed through an LSTM network and the final hidden state is $h_{L}$, where $L\text{$=$}L^{(s)}\text{$+$}L^{(p)}\text{$+$}L^{(o)}\text{$+$}2$ is the length of $n^{(r)}$.
Finally, all the above feature vectors are concatenated and passed through a fully connected neural layer to be the relation encoding vector $e^{(r)}$:
\begin{align}
    &[h_0 ... h_{L}] = \text{LSTM}(n^{(r)}) ,\\
    &e^{(r)} = \mathrm{tanh}(W[f^{(s)}, f^{(p)}, f^{(o)}, h_{L}] + b) .
\end{align}

\subsection{Decoder} 
At each decoding time step, the decoder generates either a word from the vocabulary, or a placeholders corresponding to an entity in the query graph.

Before introducing the placeholder generation strategy, we first clarify how we implement a standard LSTM decoder with attention \cite{bahdanau2014neural} over relation triples. A coverage mechanism \cite{see2017get} is also employed to encourage the decoder to generate tokens in a way such that all relation triples can be covered. The hidden states of the decoder LSTM are initialized by those of the root node from the Tree-LSTM encoder.
At time step $t$:\fromJ{I think in the case of LSTM \textbf{decoder}, it is t-1}
\begin{align}
    h_t &= \mathrm{LSTMCell}^{(d)}(x_{t-1}, h_{t-1}) ,\\
    % e_{tj} &= w^{T} \mathrm{tanh}(W[h_t, r^\mathrm{enc}_j, c_{tj}]+b) ,\\
    % a_{tj} &= \mathrm{exp}(e_{tj}) / \textstyle\sum_{k} \mathrm{exp}(e_{tk}) ,\\
    c_{tj} &= \textstyle\sum_{t'=0}^{t-1}a_{t'j}, \\
    a_{tj} &\propto w^{T} \mathrm{tanh}(W[h_t, e^{(r)}_j, c_{tj}]+b) ,\\
    r^*_t &= \textstyle\sum_{j} a_{tj} e^{(r)}_j ,
\end{align}
where $h_{t}$ is the previous hidden state of the decoder LSTM, $x_{t-1}$ is the word embedding of the previously generated token, $a_{tj}$ ($c_{tj}$) is the attention (coverage) on relation $r_j$ at time step $t$, and $r^*_t$ is the context vector. The probability distribution of words in the vocabulary to be generated is: 
\begin{equation}
\label{eq:p_vocab}
    P_\text{vocab} = \mathrm{softmax}(W[h_t, r^*_t] + b).
\end{equation}

\noindent\textbf{A new placeholder generation strategy:}
Placeholders cannot be generated in the same way as vocabulary words, because they represent different entities in different query graphs and do not have a global meaning. Observing that each relation triple contains at most one grounded entity, we design a new placeholder generation strategy by reusing the attention over relation triples.
The decoder uses a soft switch $p_\text{ph}\in[0,1]$ to  interpolate the probability of generating a placeholder and a word from the vocabulary:
\begin{align}
    &p_\text{ph} = \sigma(W[x_t, h_t, r^*_t] + b) , \label{eq:p_ph}\\
    % &P(w | w\text{$\in$}\text{vocab}) = (1 - p_\text{ph}) P_\text{vocab}(w) , \label{eq:prob_vocab} \\
    % &P(w | w\text{$=$}\text{ph}(r_j)) = p_\text{ph} \alpha'_{tj}. \label{eq:prob_placeholder} \\
    &P(w)\text{$=$}
    \begin{cases}
        (1\text{$-$}p_\text{ph}) P_\text{vocab}(w) & w\text{$\in$}\text{vocab} \label{eq:prob_vocab} \\
        p_\text{ph} \alpha'_{tj} & w\text{$=$}\text{ph}(r_j) \label{eq:prob_placeholder}
    \end{cases}.
\end{align}
Note that the attention $\alpha_{ij}'$ here differs from $\alpha_{ij}$ in that it is the softmax over only those relations containing a grounded entity rather than all the relations.

\subsection{Training}
\label{sec:t2s_train}
The model can be trained with Maximum Likelihood Estimation to optimize the probability of generating the ground truth token $w^*$, i.e. $P(w^*)$ from Eq.\ref{eq:prob_placeholder}, at each time step.
We also add a coverage loss $\mathcal{L}_\text{COV}$ to encourage attending over all the relations and a L2 regularizer:
\begin{align}
    % &\mathcal{L}_\mathrm{MSE} = \begin{cases}
    %     -log(P_\text{vocab}(w^*)),&\text{ $w^*\text{$\in$}\text{vocab}$} \\
    %     -log(P_\text{ph}(w^*))),&\text{ $w^*$=$\text{ph}(o_j)$}
    %     \end{cases} ,\\
    &\mathcal{L}_\text{MSE} = -\text{log}(P(w^*)), \\
    &\mathcal{L}_\text{COV} = \textstyle\sum_{j} \text{min}(a_{tj}, c_{tj}) ,\\
    &\mathcal{L} = \mathcal{L}_\text{MSE} + \lambda_1 \mathcal{L}_\text{COV} + \lambda_1 L2 .
\end{align}





==> sections/model_subquestions.tex <==
\section{\textsf{\small CoGSub2Q}: Sub-question Aided CQG}
\label{sec:subq-cqg}
\nop{The Tree2Seq model is made generic enough to handle all types of query graphs.
However, this one-size-fit-all solution may not be optimum, especial when the training signals become sparse as the complexity of query graphs increase. 
On the other hand, humans can handle complex sentences composition easily and naturally by thinking of simpler expressions first that can be used towards the complex sentences.
Similarly, a better CQG system should be aided by simpler sub-questions, which could be acquired either from higher-quality generation or directly retrieved from the web or from existing datasets.
We focus on the later case in this paper, and specifically investigate how to leverage associated sub-questions from WebQ and unassociated simple questions from SimpQ to aid the CQG task.
}
%\subsection{Incorporate Sub-questions}
\label{sec:incorp-subq}
One straightforward way to utilize sub-questions {(Def.\ref{def:subq})} of a given query graph is to use them for data augmentation, i.e., as additional training samples to train our \textsf{\small CoG2Q} model. However, this strategy does not fully utilize the intrinsic connections within the datasets: It can only rely on the trained parameters contributed by all the sub-questions (\emph{model-level} connection), but does not directly utilize the sub-questions corresponding to a complex query graph when generating a complex question (\emph{instance-level} connection).
\nop{The straightforward way of incorporating sub-questions is to use them as additional training samples to train the Tree2Seq, but it does not fully utilize the association relations: the model only relies on its trained parameters on all the sub-questions, but not directly from the the sub-questions of the to be generated complex questions.
In fact, such sub-question relations are easy to find by matching two query graphs.
}

Therefore, we propose to explicitly consider sub-questions as extra inputs in the generation process, and extend our \textsf{\small CoG2Q} model with a sub-question encoder and a copying mechanism \cite{see2017get} in the decoder.
\nop{Specifically, we extend our \textsf{\small CoG2Q} model with a seq2seq model with a copying mechanism \cite{see2017get} that takes a sub-question as an extra input.} We refer to this model as \textsf{\small CoGSub2Q}. After encoding a given query graph and a sub-question, the decoder in \textsf{\small CoGSub2Q} generates from an interpolated probability distribution of sub-question words, vocabulary words and placeholders.
More concretely, a sub-question token sequence $[z_1 ... z_N]$ is encoded by an LSTM encoder into vector representations $[h^{(Q)}_1 ... h^{(Q)}_N]$, and then an attention mechanism is applied over them, excluding $h^{(Q)}_i$ if $z_i$ is a placecholder:
\fromJ{Keep subscript $^\text{(Q)}$?, $h$ with and without the subscripts are different.}
\begin{align}
    &[h^\text{(Q)}_0...h^\text{(Q)}_N] = \mathrm{LSTM}^\text{(Q)}[z_0  ... z_{N}] , \label{eq:enc-subq} \\
    % e^\text{(q)}_{tj} &= w^T\text{tanh}(W[h_t, h^\text{(q)}_j] + b) ,\\
    % a^\text{(q)}_{tj} &= \text{exp}(e^\text{(q)}_{tj})/\textstyle\sum_{k}\text{exp}(e^\text{(q)}_{tk}) ,\\
    &a^\text{(Q)}_{tj} \propto w^T\text{tanh}(W[h_t, h^\text{(Q)}_j] + b) , \label{eq:attn_over_subq}\\
    &h^{\text{(Q)}*}_t = \textstyle\sum_{j}a^\text{(Q)}_{tj}h^\text{(Q)}_j .
\end{align}
Intuitively, a complex question may reuse the expressions in a sub-question, so we allow our model to directly copy words from a sub-question when generating a complex question.
We define $p_\text{copy}$ as the probability of copying a word from a sub-question rather than generating it from the entire vocabulary. 
The new $P'_\text{vocab}$ and $p'_{ph}$ are computed similarly to previous (Eqn.\ref{eq:p_vocab}-\ref{eq:p_ph}), but with the context vector $h^{\text{(Q)}*}_t$ as an additional input:
\begin{align}
    p_\text{copy} &= \sigma(W[x_t, h_j, h^{\text{(Q)}*}_t] + b) , \label{eq:p_copy} \\
    p'_\text{ph} &= \sigma(W[x_t, h_t, r^*_t, h^{\text{(Q)}*}_t] + b) , \label{eq:p_ph_prim} \\
    P'_\text{vocab} &= \text{softmax}(W[h_t, r^*_t, h^{\text{(Q)}*}_t] + b) . \label{eq:p_vocab_prim}
\end{align}
The probability of generating a word from the vocabulary is the sum of directly generating it from the vocabulary and copying it from the sub-question in which it appears:
\begin{align}
    \label{eq:p_vocab_prim_prim}
    \begin{split}
    P_\text{vocab+copy}(w) &= (1-p_\text{copy})P'_\text{vocab}(w) + \\ 
    &\qquad p_\text{copy}\textstyle\sum_{j:z_j=w}a^\text{(Q)}_{tj} .
    \end{split}
\end{align}
% \fromH{should we use capital $P_{vocab}$ or keep consistent with other prob.?} \fromJ{I kind of imitated the equations in \cite{see2017get}, my understanding is that lower case $p$ is a scalar and upper case $P$ is a probability distribution.}
The other parts of the model are the same as \textsf{\small CoG2Q}, including the attention over relations, how placeholders are generated and how to train and test the model:
\begin{align}
    &P(w)\text{$=$}
    \begin{cases}
        (1\text{$-$}p_\text{ph}) P_\text{vocab+copy}(w) & w\text{$\in$}\text{vocab} \\
        p_\text{ph} \alpha'_{tj} & w\text{$=$}\text{ph}(r_j)
    \end{cases}.
\end{align}
% \add{I think in here as well as next section, we might be better off if adding the final equation p(w*) with the new P'' and then readers might be able to directly connect to the training part in previous section. }

Based on the discussion of WebQ and CompQ in Section \ref{sec:dataset}, there is a one-to-one correspondence between a complex question and a sub-question, as the annotators for CompQ refers to a sub-question while composing a complex question.
\nop{as the annotators for ComplexQ have access to the sub-questions while composing the complex questions.}
We assume this information is known during the training phase and train \textsf{\small CoGSub2Q} in the same way as described in Section~\ref{sec:t2s_train}.
At testing time, for a given complex query graph in CompQ, we randomly sample one of its \add{(pseudo)}\fromJ{If being precise, the sampled one may be a sub-question or a pseudo.} sub-questions (if there are many), use the trained \textsf{\small CoGSub2Q} model to generate a complex question and evaluate its quality with multiple ground-truth questions as references.

% \fromH{There might be many sub-questions for a complex query graph, because you replace entities with placeholders, right?} %\fromH{Here, based on our discussion this morning, you only have one sub-question for each complexQ, right? What do you mean by "multiple ground-truth" questions? In fact, I suggest we simplify the story by only stating: base, SubQ (with association, and you can assume associating in the testing time), P-SubQ with simple questions (with random sampling for training v.s. with multiple simple questions). I feel this makes the story more clear. In the last case we explore if we do not have sub-questions available, what we should do. Randomly using a simple question does not work and hence you propose a new model.}

\nop{
\fromH{I would suggest we remove Section 6.1 and have the above paragraph.}
\subsection{Training with association}
Section~\ref{sec:t2s_train} \st{introduced how to train T2S, where the target tokens are from randomly sampled ground-truth complex questions.
Training of T/S2S additionally require the selection of a sub-question.
Basically there are two ways of choosing the sub-question for training: \emph{associated} and \emph{unassociated}.
Interestingly, experiments show that this subtle difference between sub-question selection methods plays a key role in the success of T/S2S.}

\st{Although questions with the same query-graph after placeholder replacement are grouped together for more accurate evaluation, there is still the underlying one-to-one association between a complex question and a sub-question reflecting that they are originally generated from some shared grounded entities, and the annotators have access to the sub-questions while composing the complex questions.
The associated training strategy differs from the unassociated in that it choose the sub-question associated with the randomly sampled target complex question rather than randomly sample sub-question as well.
Note that such associations are not assumed during testing: we randomly sample a sub-question, use the model to generate a complex question and evaluate its quality with the multiple ground-truth questions.}
}



==> sections/model_subquestions_multi.tex <==
\section{\textsf{\small CoGSub$^m$2Q}: CQG with Multiple Pseudo Sub-Questions}
\label{sec:pseudo-subq-cpq}
In reality, given a query graph, its corresponding sub-questions {(Def.\ref{def:subq})} may not be available. However, there already exist large-scale simple question datasets such as SimpQ {discussed in Section~\ref{sec:dataset}, and moreover, simple questions can be easily harvested from user queries, chat logs, etc}.
We can treat simple questions as pseudo sub-questions (Def.\ref{def:pseudo-subq}) for a complex query graph as long as the predicate in the former appears in the latter.
In this section, {we explore how to leverage pseudo sub-questions to help CQG, in the scenario where sub-questions are not available.}
\nop{Although sometimes like in the last section, we are lucky to have associated sub-questions for CQG, this may not always be the case when one is dealing with a new KG.
So in this section, we further explore the followup question: without the associated sub-questions, can simple questions still be able to aid CQG?

Unassociated simple questions can be easily accessible.
Both human annotating or automatic generating simple questions are relatively easier, and they can be retrieved from 
the web (e.g. using search APIs \cite{}) with the help of other techniques (e.g. relation extraction \cite{}).
We use the SimpQ dataset for the study of this task, because it is separately curated from CompQ so there are no sub-question associations as in WebQ, as discussed in Section~\ref{sec:dataset}.
It is also at a much larger scale than WebQ, thus has the potential to contain some simple questions that can help complex question generation.
}
% We put it as a future work to study the case where SimpleQuestions do not cover any relations in the complex query graph.
% However, even for those cases, one can leverage either the existing work \cite{serban2016generating, elsahar2018zero} to generate the needed simple questions, or borrow distant supervision acquire methods in relation extraction to find some useful text snippets from the web that are very close to a single-relation question.
\nop{
\subsection{Pseudo-associated simple questions}
\fromH{I suggest we remove this section, and directly propose the model for ranking multiple simple questions.}}
\nop{We hypothesis that one of the reasons why associations are important to training the T/S2S model is because the associated sub-questions and the questions share more words or phrases in common, so the model can easily learn to decode the complex question based on the sub-question encoding or directly copy words from it.
On the other hand, learning from unassociated sub-questions can be much more difficult because the model has to deal with more paraphrases.

Follow this intuition, we then propose to find the \emph{pseudo-associated} simple questions as those having more word overlaps with the complex question.
Specifically, we first find for each complex question all the simple questions that shares a relation with it, then pick those with the highest BLEU scores with it as the pseudo-associated simple questions. 
Therefore we can do the same experiments as in the previous section.
If the pseudo-associations have the same quality as real ones, utilizing the simple questions may leads to similar performance improvements at test time.
}

%\subsection{Utilizing multiple simple questions}
% \add{One intuitive way to utilize SimpQ for CQG is to randomly sample a pseudo sub-question for a given query graph and then train the \textsf{\small CoGSub2Q} model as before. Our experiments will show that .. We hypothesize that this is because XX  and also verify this via a simulation experiment (details in Section ..).   \fromH{if we do not have space, we might remove this..}}

Since we usually can find multiple pseudo sub-questions for a given query graph, we further extend \textsf{\small CoGSub2Q} to automatically learn which pseudo sub-question is better associated with the query graph and can be more helpful for generating the ground-truth question. 
% \nop{Since it is easier to find more simple question, we extend the T/S2S model to be able to utilize multiple simple questions while learning which one is more associated.}
% \nop{It is also more flexible to let the model automatically learn the association scores of pseudo sub-questions rather than use prefixed ones.
% The model can be more robust at test time, as it leverages more than one simple questions.} 
We refer to this model as \textsf{\small CoGSub$^m$2Q}.
Formally, given a set of $M$ simple questions $\{[z^m_1...z^m_{N^m}]\}_{m \in [1:M]}$, each of them is used independently to calculate the  $a^\text{(Q)}_{tj}$, $p'_{ph}$, $P''_\text{vocab}$ and $P(w)$ as before in Section~\ref{sec:subq-cqg} (Eqn.\ref{eq:attn_over_subq},\ref{eq:p_ph_prim},\ref{eq:p_vocab_prim_prim} and \ref{eq:prob_placeholder}). We use $P_m(w)$ to represent the generation probability for the $m$-th pseudo sub-question.

We then define a two-level attention score for each simple question:
First, $a_{jm}$ is the attention over the $j$-th word in the $m$-th simple questions, computed with the simple question encoding $[h^{(Q)m}_1...h^{(Q)m}_{N^m}]$ (Eq.\ref{eq:enc-subq}) and the encoding of the query tree at root $h^{\text{(T)}m}_{root}$ (Eq.\ref{eq:tree-lstm}).
Then, $a_m$ is the attention for the $m$-th simple question as a whole, computed by the attentive aggregation of simple question word encoding and the query tree root encoding. Formally:
\begin{align}
    % e_{tm} &= Wh^{(n)m}_t ,\\
    % a_{tm} &= \text{exp}(e_{tm}) / \textstyle\sum_{m'}\text{exp}(e_{tm'}) ,\\
    a_{jm} &\propto W [h^{\text{(Q)}_m}_j, h^{\text{(T)}_m}_{root}] , \\
    % e_{m} &= W\textstyle\sum_t a_{tm}h^{(n)m}_t ,\\
    % a_{m} &= \text{exp}(e_{m}) / \textstyle\sum_{m'}\text{exp}(e_{m'}) .
    h^{\text{(Q)}_m*} &= \textstyle\sum_j a_{jm}h^{\text{(Q)}_m}_{j} , \\
    % a_{m} &\propto W [\textstyle\sum_j a_{jm}h^{(Q)m}_{j}, h^{\text{(T)}m}_{root}] .
    a_{m} &\propto W [h^{\text{(Q)}_m*}_{j}, h^{\text{(T)}_m}_{root}] .
\end{align}
% The first two equations above attend over the words in each simple question, and the last two equations above attend over a simple question as a whole.
The learned association scores can be used to compute the weighted average for generating vocabulary words or placeholders. Specifically:
\begin{align}
    % &\bar{P}''_\text{vocab}(w) = \textstyle\sum_m a_m P''^m_\text{vocab}(w) , \\
    % \begin{split}
    % \bar{P}(w) = &\textstyle\sum_m a_m P^{m}(w), \\
    % & w \text{$\in$}vocab \ \ \text{or}\ \ w \text{$=$} \text{ph}(o_j) .
    % \end{split}
    \bar{P}(w) = \textstyle\sum_m a_m P_m(w).
\end{align}

% \noindent\textbf{Training.}
% \fromH{This strategy seems not well explained (please also see my related comments in exp)..I think we can start with ``The most intuitive way to buld the set of pseudo sub-questions is via random sampling.. however, we observe not effective (to be shown in exp..). Noticing that.. we propose to include the one with highest BLEU in training (Alternatively, THIS STRATEGY can be mentioned in exp rather than here)..''} 
% During training, we build the set of simple questions with the simple question with the highest BLEU and the others are randomly sampled.
% During testing, all the simple questions are randomly sampled.
% This training strategy not only allows the model to easily learn from simple questions with the most word overlaps, and also leaves it the flexibility to choose simple question on it own.

==> tables_new/compare_using_multiple_subquestions_less.tex <==
\begin{table}[t!]
% \small
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{@{}p{0.2cm}p{2.3cm}lll@{}}
\toprule
&                                   & \textbf{BLEU-4} & $\text{\textbf{ROUGE}}_\text{\textbf{L}}$   & \textbf{METEOR}    \\ 
% \midrule
\toprule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{{\textbf{w/ sub-q}}}}}
&\textsf{\small CoG2Q}          & 28.68 & 51.83                     & 37.54     \\\cmidrule{2-5}
&\textsf{\small CoG2Q} + data   & 29.23 & 52.64                     & 38.33     \\ 
&\textsf{\small CoGSub2Q}*      & 29.23$\pm$0.14 & 52.68$\pm$0.12 & 37.98$\pm$0.12     \\  
&\textsf{\small CoGSub2Q}       & \textbf{31.43}$\pm$0.13 & \textbf{55.26}$\pm$0.13 & \textbf{39.77}$\pm$0.06     \\ \midrule\midrule

\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{{\textbf{w/ pseudo}}}}}
&\textsf{\small CoG2Q}          & 27.89 & 51.62                     & 36.50     \\ 
\cmidrule{2-5}
&\textsf{\small CoG2Q} + data   & 28.87 & 52.35                     & 37.83     \\
&\textsf{\small CoGSub2Q}*      & 29.58$\pm$0.13 & 52.94$\pm$0.14 & 38.02$\pm$0.05 \\  
% &\textsf{\small CogSub2Q} (train w/ assoc.) & 29.18$\pm$0.10 & 52.25$\pm$0.17 & 37.90$\pm$0.14 \\ 
\cmidrule{2-5}
% &\textsf{\small CogSub$^m$2Q} (train w/ rand.)  & 61.37$\pm$0.16 & 46.02$\pm$0.13 & 36.29$\pm$0.09 & 30.12$\pm$0.07 & 53.45$\pm$0.09 & 38.05$\pm$0.07 \\
&\textsf{\small CoGSub$^m$2Q}   & \textbf{30.95}$\pm$0.19 & \textbf{53.68}$\pm$0.10 & \textbf{38.74}$\pm$0.05 \\
\bottomrule
\end{tabular}
}
\caption{Complex question generation with sub-questions from WebQuestionsSP (upper-half) and multiple pseudo sub-questions from SimpleQuestions (lower-half). &\textsf{\small CoGSub2Q}* with a asterisk indicates that the model is trained with pseudo sub-questions rather than actual sub-questions.}
\label{tab:compare_using_multiple_subquestions_less}
\end{table}


==> tables_new/datastats.tex <==
\begin{table}[t]
\centering
\small
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{@{}crrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{No. query}\\\textbf{graphs}\end{tabular}} & \multicolumn{3}{r}{\textbf{No. ques. per query graph}} \\
\cmidrule{3-5}
% \cline{3-5}
        &           & \textbf{\footnotesize Median}    & \textbf{\footnotesize Average}       & \textbf{\footnotesize Max}       \\ \midrule 
WebQ    & 585       & 2         & 7         & 185       \\
SimpQ   & 441       & 20        & 178       & 3,810     \\
CompQ   & 6,162     & 2         & 4         & 136       \\
\bottomrule
\end{tabular}
}
\caption{Dataset statistic. For all three datasets, numbers of examples reduce substantially after merging, and numbers of questions per example are highly screwed. SimpQ has only 441 relations that appears in CompQ, out of 1,837 in total.}
\label{tab:data_stats}
\end{table}
